On Finding Local Nash Equilibria (and Only Local Nash Equilibria) in Zero-Sum Games

We propose local symplectic surgery, a two-timescale procedure for finding local Nash equilibria in two-player zero-sum games. We first show that previous gradient-based algorithms cannot guarantee convergence to local Nash equilibria due to the existence of non-Nash stationary points. By taking advantage of the differential structure of the game, we construct an algorithm for which the local Nash equilibria are the only attracting fixed points. We also show that the algorithm exhibits no oscillatory behaviors in neighborhoods of equilibria and show that it has the same per-iteration complexity as other recently proposed algorithms. We conclude by validating the algorithm on two numerical examples: a toy example with multiple Nash equilibria and a non-Nash equilibrium, and the training of a small generative adversarial network (GAN).

==> conc_bnd.tex <==
% !TEX root = JMLR18.tex

Having shown that \eqref{eq:TTSsys} has the desired asymptotic behavior, we now investigate its non-asymptotic rate of convergence. We relax our assumptions on the function, noise, and stepsizes from the previous section to derive an upper bound on the \emph{lock-in} probability of \eqref{eq:TTSsys}. The \emph{lock-in} probability of a stochastic approximation can be thought of as a conditional probability of staying in a given region of the parameter space for all time given that you enter it at a certain time. The process, is thus considered to be `locked in' to this region of the state space. We note that, without making further assumptions on the cost function $f$, the only place we can analyze the behavior of \eqref{eq:TTSsys}, is in regions of attractions of LASE, where the function is well understood. Therefore, we analyze the lock-in probability of the two-timescale process around LASE.  The high-probability bound also serves as a high probability rate of convergence of the process to LASE in regions around such an equilibrium. We note that when there is a globally asymptotically stable equilibrium, our result would hold globally throughout the state space. 

% To begin, let $z^*$ be a LASE, of the dynamics \eqref{eq:ctalg}. From Proposition~\ref{prop:jac}, $z^*$ must be a DNE of the game $\mc{G}$.  By a converse Lyapunov theorem (see \cite{ConverseLyap}) there exists a Lyapunov function $V:\mb{R}^d\rar \mb{R}$ such that $V(z^*)=0$, $V(z)>0$, $\nabla V(z)\dot h(z)<0$ for all $z \in U$, for $U\subset \X$. When the process is initialized in $U$ and follows the deterministic flow $\dot z=-h(z)$, the Lyapunov function guarantees exponentially fast convergence to $z^*$. Let $R_z$ be the radius of the largest ball, centered at $z^*$ such that $B_{R_z}(z^*) \subset U$. 

%Let$\lambda_n$ be the minimum eigenvalue of the symmetric matrix $J_h(z^*)$. We know from Proposition~\ref{prop:jac}, that $\lambda_n>0$.  Since $J_h(z^*)$ is symmetric we also know that $||exp(-Dh(z^*))||\le exp(-\lambda_n)$. 


To begin we state our relaxed assumptions on the process. These relaxed assumptions apply to the vast majority of settings, and allow us to analyze the behavior of our algorithm around LASE under realistic conditions. 


We begin by stating our assumptions on the function, the estimator, and the step-sizes. We remark that these assumptions are more relaxed than what has been considered before in the literature on two-time scale processes, and are most similar to the conditions assumed for single time-scale processes analyzed in \cite{Borkar:Alekseev}. We first make some assumptions on the function $f$.

\begin{assumption}{Assumptions on $f$:}
Assume that $f \in \mc{C}^n(:\mb{R}^d,\mb{R} $ for $n\ge3$.
\label{ass:f}
\end{assumption}

Given that we now allow $J$ to be singular, for a fixed $z$, $v^*(z)=J^{\dagger}(z)\omega(z)$, where $J^{\dagger}(z)$ is the pseudo-inverse of $J$. Since it is not clear that the LASE of $h_1(z,v^*(z))$ are still only the DNE of $\mc{G}$ we show, in Appendix \ref{app:proof_pseudo}, that the findings of Proposition \ref{prop:jac} still hold.

We now state our assumptions on the sequence of step-sizes $a_n$ and $b_n$. We remark that we do not require either sequence to be square-summable, which is a significant departure from previous work, and allows us to apply our results to more realistic settings.

\begin{assumption}{Assumptions on the step-sizes:}
We assume that $f \in C^n$ for $n\ge2$. Then, since $B_{R_z}(z^*)$ is compact, both $\omega$ and $J$ must satisfy:
\begin{itemize}
	\item $\lim_{n\rar \infty} a_n=0$, and $\lim_{n\rar \infty} b_n=0$.
	\item $\sum_{i=1}^\infty a_i=\infty$, and  $\sum_{i=1}^\infty a_i=\infty$.
	\item $\sup_{n\ge1} a_i \le 1$, and $\sup_{n\ge1} b_n \le 1$.
\end{itemize}
Finally we assume that the sequence $a_n$ decreases faster than $b_n$:  $\lim_{n \rar \infty} \frac{a_n}{b_n}=0$.
\label{ass:ss}
\end{assumption}

Next, we make assumptions on the noise. We note again that this is a relaxation of Assumption~\ref{ass:noise}, and this allows us to consider a general class on the noise processes.

\begin{assumption}{Assumptions on the noise:}
We first define the filtration $\mc{F}_n$, $\mc{F}_n=\sigma(z_0,v_0,M^v_1,M^z_1,...,M^z_n,M^v_n)$ for $n\ge$. Given $\mc{F}_n$, we assume that:
\begin{itemize}
	\item $M_{n+1}^v$ and $M_{n+1}^z$ are conditionally independent given $\mc{F}_{n}$ for $n\ge0$.
	\item $\mb{E}[M_{n+1}^v|\mc{F}_n]=0$ and $\mb{E}[M_{n+1}^z|\mc{F}_n]=0$ for $n\ge0$.
	\item $Pr(M_{n+1}^z>u|\mc{F}_n)\le c_1(z_n) e^{-c_2(z_n)u}$ and $Pr(M_{n+1}^v>u|\mc{F}_n)\le c_3(z_n) e^{-c_4(z_n)u}$ for $c_1,c_2,c_3,c_4>0$ and $u\ge \bar u>0$ for $\bar u$ sufficiently large.
\end{itemize}
\label{ass:noise2}
\end{assumption}

We remark that the distribution of the noise only depends on $z_n$ since $J$ and $\omega$ are the only objects that introduce randomness to the process and neither of them depend on $v$.

Finally we assume that there exists, $z^*$ a LASE, of the dynamics \eqref{eq:ctalg}. From Proposition~\ref{prop:jac}, $z^*$ must be a DNE of the game $\mc{G}$.  By a converse Lyapunov theorem (see \cite{ConverseLyap}) there exists a Lyapunov function $V:\mb{R}^d\rar \mb{R}$ such that $V(z^*)=0$, $V(z)>0$, $\nabla V(z)\dot h(z)<0$ for all $z \in U$, for $U\subset \X$. When the process is initialized in $U$ and follows the deterministic flow $\dot z=-h(z)$, the Lyapunov function guarantees exponentially fast convergence to $z^*$. Let $R_z$ be the radius of the largest ball, centered at $z^*$ such that $B_{R_z}(z^*) \subset U$. 


\begin{theorem}
Let $R_0^z>0$ be a positive constant such that $R_z>R_0^z>0$. Further pick an $\epsilon>0$ such that $\epsilon<R_0^z$. Finally let $n_0\ge N_0$ for $N_0\equiv N_0(a_n,b_n,\epsilon,R^z)$, and $n_1\ge N_1$ for $N_1\equiv(n_0,a_n,b_n,\epsilon,R^z)$. Then there exists positive constants $K_1,K_2,K_3,K_4$ such that:

\begin{align*} 
&Pr(||z_{n}-z^*||\le \epsilon \ \ ,\ \ ||v_{n}-v^*(z_n)||\le R^v \ \ \forall n\ge n_1 \ \ | \ \ ||z_{n_0}-z^*||\le R_0^z)\ge \\
 &\ \ \ \ \ \ \ 1-c_1\sum_{n=n_0}^\infty \left[exp\left(-K_1\frac{\sqrt{\epsilon}}{\sqrt{a_n}}\right)+exp\left(-K_2\frac{\epsilon^2b_n}{a_n}\right)\right]\\
 &\ \ \ \ \ \ \ \ \ \ \ \ -2d^2\sum_{n=n_0}^\infty \left[exp\left(-K_3\frac{\epsilon^2}{a_n}\right)+exp\left(-K_4\frac{\epsilon^2}{b_n}\right)\right]
\end{align*}

Where $R^v$ is an arbitrary constant such that $R^v\ge||v_{n_0}-v^*(z_{n_0})||$.
\label{thm:concbnd}
\end{theorem}

The proof for \ref{thm:concbnd} is supplied in Appendix~\ref{app:conc_pf}. It makes use of a method of deriving convergence rates for stochastic approximations by using Alekseev's formula to view the noise and the fast timescale as perturbations to the limiting ode. This method was first introduced in \cite{Borkar:Alekseev} for single time-scale stochastic approximation, and was applied to linear two-timescale processes in \cite{TTSConc1} and to more general situations in \cite{Borkar:TTS}. We note however that \cite{Borkar:TTS} still requires the square-summability of the step-sizes and assumes global asymptotic stability of the LASE of the slow process. We relax both of these assumptions.   

If we assume that $a_n=1/(1+n)^\alpha$, and $b_n=1/(1+n)^{\alpha/2}$, where $0<\alpha<1$. The following lemma gives us a more digestible rate of convergence.

\begin{lemma}
Let $R_0^z>0$ be a positive constant such that $R_z>R_0^z>0$. Further pick an $\epsilon>0$ such that $\epsilon<R_0^z$. Finally let $n_0\ge N_0$ for $N_0\equiv N_0(a_n,b_n,\epsilon,R^z)$, and $n_1\ge N_1$ for $N_1\equiv(n_0,a_n,b_n,\epsilon,R^z)$. Then if $a_n=1/(1+n)^\alpha$, and $b_n=1/(1+n)^{\alpha/2}$, where $0<\alpha<1$:
\begin{align*} 
Pr(||z_{n}-z^*||\le \epsilon \ \ ,\ \ ||v_{n}-v^*(z_n)||\le R^v \ \ \forall n\ge n_1 \ \ | \ \ ||z&_{n_0}-z^*||\le R_0^z)\ge\\
 &  \ \ \ \ 1-O\left(n_0^{1-\alpha/2}e^{-Cn_0^{\alpha/2}}\right)
\end{align*}

Where $R^v$ is an arbitrary constant such that $R^v\ge||v_{n_0}-v^*(z_{n_0})||$.
\label{lemma:Obnd}
\end{lemma} 

We note that the bound in the previous lemma is on the same order as that of \cite{Borkar:Alekseev}, which implies that the two-timescale approximation has convergence on the same order as a single-timescale process with similar assumptions on the noise and stepsize. The proof of Lemma \ref{lemma:Obnd} is supplied in Appendix~\ref{app:conc_pf}.

The bound in Theorem~\ref{thm:concbnd} assures us that even under relaxed conditions on the stepsizes, loss function, and estimators, the two-timescale approximation \eqref{eq:TTSsys} will converge in high probability to a LASE if it reaches its region of attraction. Further, the finite time rate of convergence is comparable to that of a single-timescale process having  the same step-size as the slow timescale. Thus, around LASE, the number of iterations for convergence of the two-timescale process \eqref{eq:TTSsys} is on the same order as that of the single-timescale variant \eqref{eq:dtalg}, but in practice it may be faster due to the fact that we do not need to invert a matrix.



==> thm.tex <==
% !TEX root = JMLR18.tex
% \subsection{Setup and Assumptions} 
First, let $z^*$ be a LASE, of the desired dynamics $h$. By a converse Lyapunov Theorem \tc{red}{CITE CONVERSE LYAP} there exists a Lyapunov function $V$ such that $V(z^*)=0$, $V(z)>0$, $\nabla V(z)\dot h(z)<0$ for all $z \in U$, for $U\subset \X$. Let $R_z$ be the radius of the largest ball, centered at $z^*$ such that $B_{R_z}(z^*) \subset U$. We note that $Dh(z^*)$ has strictly positive eigenvalues from \tc{red}{CITE First thm}. Let $\lambda_n=Re(\lambda_{min}(Dh(z^*)))$. Now since $Dh(z^*)$ is symmetric, for all $\kappa \in (0,1)$, and defining $\lambda'=\kappa \lambda_n$, we know that $||exp(-Dh(z^*))||\le exp(-\lambda')$. 

We begin by stating our assumptions on the function, the estimator, and the step-sizes. We remark that these assumptions are more relaxed than what has been considered before in the literature on two-time scale processes, and are most similar to the conditions assumed for single time-scale processes analyzed in \tc{red}{CITE ALEKSEEV FORMULA}. We first make some assumptions on the function $f$.

\begin{assumption}{Assumptions on $f$:}
We assume that $f:\mb{R}^d\rar\mb{R} \in C^n$ for $n\ge2$. Then, since $B_{R_z}(z^*)$ is compact, both $\omega$ and $J$ must satisfy:
\begin{itemize}
	\item $f$ is $L_f$-Lipschitz continuous on $B_{R_z}(z^*)$.
	\item $\omega:\mb{R}^d\rar \mb{R}^d$ is $L_\omega$-Lipschitz continuous on $B_{R_z}(z^*)$.
	\item $J:\mb{R}^d \rar \mb{R}^{d\times d} $ is $L_J$-Lipschitz continuous on $B_{R_z}(z^*)$.
\end{itemize}
We further assume that $||J(z)||>\sigma_{min}>0 \ \ \forall \ \  z \in B_{R_z}(z^*)$ and define $\sigma_{max}=\max_{z \in B_{R_z}(z^*)} ||J(z)||$.
\label{ass:f}
\end{assumption}

We now state our assumptions on the sequence of step-sizes $a_n$ and $b_n$. We remark that we do not require either sequence to be square-summable.
\begin{assumption}{Assumptions on the step-sizes:}
We assume that $f \in C^n$ for $n\ge2$. Then, since $B_{R_z}(z^*)$ is compact, both $\omega$ and $J$ must satisfy:
\begin{itemize}
	\item $\lim_{n\rar \infty} a_n=0$, and $\lim_{n\rar \infty} b_n=0$.
	\item $\sum_{i=1}^\infty a_i=\infty$, and  $\sum_{i=1}^\infty a_i=\infty$.
	\item $\sup_{n\ge1} a_i \le 1$, and $\sup_{n\ge1} b_n \le 1$.
\end{itemize}
Finally we assume that the sequence $a_n$ decreases faster than $b_n$:  $\lim_{n \rar \infty} \frac{a_n}{b_n}=0$.
\label{ass:ss}
\end{assumption}

Finally we make further assumptions on the noise processes $M^z_n$, and  $M^v_n$. 

\begin{assumption}{Assumptions on the noise:}
We first define the filtration $\mc{F}_n$, $\mc{F}_n=\sigma(z_0,v_0,M^v_1,M^z_1,...,M^z_n,M^v_n)$ for $n\ge$. Given $\mc{F}_n$, we assume that:
\begin{itemize}
	\item $M_{n+1}^v$ and $M_{n+1}^z$ are conditionally independent given $\mc{F}_{n}$ for $n\ge0$.
	\item $\mb{E}[M_{n+1}^v|\mc{F}_n]=0$ and $\mb{E}[M_{n+1}^z|\mc{F}_n]=0$ for $n\ge0$.
	\item $Pr(M_{n+1}^z>u|\mc{F}_n)\le c_1 e^{-c_2u}$ and $Pr(M_{n+1}^v>u|\mc{F}_n)\le c_3 e^{-c_4u}$ for $c_1,c_2,c_3,c_4>0$ and $u\ge \bar u>0$ for $\bar u$ sufficiently large.
	%\item $||M_{n+1}^z||\le c_z(1+||z_n||)$ and $||M_{n+1}^v||\le c_v(1+||z_n||)$ almost surely.
\end{itemize}
\label{ass:noise}
\end{assumption}

We note that, in the last assumption the dependence is solely on $z_n$ due to the fact that the randomness in the process comes only from $\omega$ and $J$ which depend only on the current value of $z_n$. 

\begin{theorem}
Let R be the radius of the largest ball, centered at $z^*$, that fits in $dom(V)$, Let $R>R_1^z>R_0^z>0$. Further pick an $\epsilon$ such that $0<\epsilon<R_0^z$. Finally let $n_0=N_0(a_n,b_n,\epsilon,R_1^z)$, and $n_1=N_1(n_0,a_n,b_n,\epsilon,R_1^z)$. Then when $||z_{n_0}-z^*||\le R_0^z$ then:
\begin{align*} 
&Pr(||z_{n}-z^*||\le \epsilon,\ \ \forall n\ge n_1)\ge \\
 &\ \ \ \ \ \ \ 1-2d^2\sum_{n\ge n_0}\left[ exp\left[\frac{-C_1\sqrt{\epsilon}}{\sqrt{a_n}}\right]+exp\left[\frac{-C_2\epsilon}{a_n}\right]+exp\left[\frac{-C_3\epsilon}{b_n}\right] \right] 
\end{align*}
Where $C_1,C_2,C_3>0$ are constants depending on the parameters in the assumptions.
\label{thm:concbnd}
\end{theorem}

Before proving Theorem~\ref{thm:concbnd} we first derive a concentration bound for the fast-time scale $v_n$. To simplify our analysis, we first rewrite the fast time scale.  Let $\bar v_n=v_n-v^*_n$. Letting, $A_(z_n)=J^T(z_n)J(z_n)$, and $\Delta_{n+1}=v^*_n-v^*_{n+1}$, the update equation for $\bar v_n$ is given by:

\[ \bar v_{n+1}=\bar v_{n}-b_n[A(z_n)\bar v_n+M^v_{n+1}]+\Delta_{n+1}\]

Letting $B(z_n)=I-b_nA(z_n)$, this further simplifies to:

\[ \bar v_{n+1}=B(z_n)\bar v_n-b_n M^v_{n+1}+\Delta_{n+1}\]

The slow time-scale, as a function of $\bar v_n$ is given by:

\[z_{n+1}=z_n-a_n(h(z_n)-J^T(z_n)\bar v_n+M^z_n)\]

Letting $n_1=n_0+n+1$ we can now write:

\begin{align}
\bar v_{n_1}=&\prod_{i=n_0}^{n_0+n}B(z_i)\bar v_{n_0} \label{term:t1v}\\
&-\sum_{i=n_0}^{n_1-1}b_i\left(\prod_{j=i+1}^{n_1-1}B(z_j) \right)M^v_{i+1}\label{term:t2v}\\
&+\sum_{i=n_0}^{n_1-1}\left(\prod_{j=i+1}^{n_1-1}B(z_j)\right)\Delta_{i+1}\label{term:t3v}
\end{align}

We now define a continuous approximation to the $z_n$ process, which is found by the linear interpolation of $z_n$. Define $t_n=\sum_{i=0}^n a_n$. Then the linear interpolated process $\bar z(t)$ for $t \in [t_n,t_{n+1}]$ is given by:

\[\bar z(t)=\bar z(t_n)+\frac{t-t_n}{a_n}(\bar z (t_{n+1})-\bar z (t_n)) \]

Note, that the linear interpolation agrees with the discrete process at $t_n$ for $n\ge0$.

Thus, for any $n \ge0$:

\begin{align*}
\bar z(t)&=\bar z(t_{n_0})-\sum_{k=n_0}^n a_k (h(\bar z(t_k))+J^T(\bar z(t_k))\bar v_k+M_k^z)\\
&=\bar z(t_{n_0})-\sum_{k=n_0}^n \int_{t_k}^{t_{k+1}} [h(\bar z(t_k))+J^T(\bar z(t_k))\bar v_k+M_k^z]ds\\
&=\bar z(t_{n_0})-\int_{t_{n_0}}^{t_{n}}[ ]h(\bar z(s))+g_1(s) +g_2(s)+g_3(s)] ds
\end{align*}

Where, for $t \in [t_n,t_{n+1}]$:
\begin{align}
g_1(t)&=h(\bar z(t_{n}))-h(\bar z(t))\\
g_2(t)&=J^T(z(t_{n}))\bar v_n\\
g_3(t)&=M^z_{n+1}
\end{align}

Now, let a solution to the limiting ode, $\dot z=-h(z)$, starting at $z_0$ from $t_0$ to $t$, be given by $z(t,t_0,z_0)$. Via Alekseev's formula, we can write"

\[\bar z(t)=z(t,t_{n_0},\bar z(t_{n_0}))+\int_{t_{n_0}}^t \Phi(t,s,\bar z(s))(g_1(s)+g_2(s)+g_3(s))ds\]

Where $\Phi(t,s,\bar z(s))$ is the fundamental matrix of $\dot y=Dh(z_(t),s,u_0)y$ for $t\ge0$ where $Dh$ is the Jacobian along the trajectory of $z(t)$. Note that $g_1(s)+g_2(s)+g_3(s)$ is piece-wise continuous. 

\[\bar z(t)=z(t,t_{n_0},\bar z(t_{n_0}))+\int_{t_{n_0}}^t \Phi(t,s,\bar z(s))(g_1(s)+g_2(s)+g_3(s))ds\]

We now rewrite this as:

\[\bar z(t_n)=z(t,t_{n_0},\bar z(t_{n_0}))+W_n+S_n^z+(\tilde S_n^z-S_n)+V_n+(\tilde V_n-V_n) \]

Where:
\[ W_n=\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}\Phi(t,s,\bar z(s))[h(\bar z(t_k))-h(\bar z(s)]ds\]

\[ S^z_n=\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}\Phi(t,s,\bar z(t_k))dsM^z_k\]
\[ \tilde S^z_n=\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}\Phi(t,s,\bar z(s))dsM^z_k\]
\[ V_n=\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}\Phi(t,s,\bar z(t_k))ds \bar v_{t_k}\]
\[\tilde V_n=\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}\Phi(t,s,\bar z(s))ds \bar v_{t_k}\]


\subsection{Defining the event of interest}
The event we would like to bound is: $\{||z_n-z^*||<\epsilon \forall n\ge n_1\}$ on the event $\{||z_{n_0}-z^*||\le R_0^z\}$. where $n_1>n_0$. W will construct an upper bound on the complement of this event using the bounds we have just constructed and the martingale concentration inequality used in Lemma \ref{lemma:vconc}.

\begin{lemma}
\label{lemma:event}
\[\mc{E}^c_z(n_1)\subseteq \left[ \bigcup_{n_0\le n \le n_1} \left(\{E_{n+1}>R^z_1-R^z_0 ,G_n\}\cup \{||\bar v_{n+1}||>R^v,G_n\}\right)\right]\cup \left[ \bigcup_{n\ge n_1+1}\{E^*_{n+1}>\epsilon,||v_{n+1}||>R^v,G_n\}\right]\]
\end{lemma}

\begin{proof}
Define:
\[\mc{E}_z(n_1):=\{||\bar z(t)-z^*||<\epsilon \ \ \forall \  t\ge t_{n_1+1}\}\cap \{||\bar v_n||<R^v \ \ \forall \  n\ge n_1+1\} \]
\[ B_{R^z_1}(z^*):=\{z: ||z-z^*|| \le R^z_1\}\]
\[ B_{R^v}(0):=\{v: ||v|| \le R^v\}\]
\[ E_{n+1}:=\sup_{t \in [t_n, t_{n+1}]} || \bar z(t)-z(t,t_{n_0},\bar z(t_{n_0}))||\]
\[ E^*_{n+1}:=\sup_{t \in [t_n, t_{n+1}]} || \bar z(t)-z^*||\]
\[ G^z_n:=\{\bz(t) \in B_{R^z}(z^*) \ \forall t \in [t_{n_0},t_n]\}\]
\[ G^v_n:=\{\bar v_k \in B_{R^v}(0) ; k=n_0,...,n\}\]
\[ G^{gap}_n:=\{\sup_{n_0\le k \le n } E_{k+1} >R^z_1-R^z_0\}\]
\[ G_n=G^z_n \cap G^v_n\]
\[ D_n=G^{gap}_n \cap G^v_n\]


We would like to find a superset of $\mc{E}^c_z(n_1)$ where $n_1=n_0+N$. 

%First, note that $\mc{E}_z(n_1)=\bigcap_{n=n_1+1}^{\infty} \{ E^*_{n+1} \le \epsilon \}$. Therefore $\mc{E}^c_z(n_1)=\bigcup_{n=n_1+1}^{\infty} \{ E^*_{n+1} > \epsilon \}$. 

%Now, $\bigcup_{n=n_1+1}^{\infty} \{ E^*_{n+1} > \epsilon \} \subseteq G_{n_1}^c \cup \bigcup_{n=n_1+1}^{\infty} \{ E^*_{n+1} > \epsilon \}$


\[ \mc{E}^c_z(n_1)= (\mc{E}^c_z(n_1)\cap D_{n_1}^c)\cup(\mc{E}^c_z(n_1)\cap D_{n_1}) \subseteq D_{n_1}^c\cup(\mc{E}^c_z(n_1)\cap D_{n_1})\]

We first analyze $D_{n_1}^c$:
\begin{align*}
D_{n_1}^c&=(G^{gap}_{n_1})^c \cup (G^v_{n_1})^c\\
&=\{\sup_{n_0\le n \le n_1 }E_{n+1}>R^z_1-R^z_0\}\cup \{\sup_{n_0\le k\le n_1+1}||\bar v_k||>R^v\}\\
&=\left[(G^{gap}_{n_1})^c \cup (G^v_{n_1})^c\right] \cup \left[\left(G^{gap}_{n_1} \cap G^v_{n_1} \right) \cap \left(\{E_{n_1+1}>R^z_1-R^z_0\}\cup \{||\bar v_{n_1+1}||>R^v\}\right)\right]
\end{align*}

Doing this recursively, we get:

\begin{align*}
D_{n_1}^c&=\bigcup_{n_0\le n \le n_1}\left(G^{gap}_{n} \cap G^v_{n} \right) \cap \left(\{E_{n+1}>R^z_1-R^z_0\}\cup \{||\bar v_{n+1}||>R^v\}\right)
\end{align*}

Using the fact that $G^{gap}_n\subseteq G^z_n$: lets us write this as:

\begin{align*}
D_{n_1}^c&\subseteq\bigcup_{n_0\le n \le n_1}\left(G^{z}_{n} \cap G^v_{n} \right) \cap \left(\{E_{n+1}>R^z_1-R^z_0\}\cup \{||\bar v_{n+1}||>R^v\}\right)\\
&=\bigcup_{n_0\le n \le n_1} \left(\{E_{n+1}>R^z_1-R^z_0 ,G_n\}\cup \{||\bar v_{n+1}||>R^v,G_n\}\right)
\end{align*}

Now we analyze $(\mc{E}^c_z(n_1)\cap D_{n_1})$. Since $D_{n_1}\subseteq G_{n_1}$, we can expand this, and write:

\begin{align*}
\mc{E}^c_z(n_1)\cap D_{n_1}\subseteq \mc{E}^c_z(n_1) \cap G_{n_1} &= \bigcup_{n\ge n_1+1}\{E^*_{n+1}>\epsilon,||v_{n+1}||>R^v_1,G_n\}\\
&\subseteq\bigcup_{n\ge n_1+1}\{E^*_{n+1}>\epsilon,G_n\}\cup\{||v_{n+1}||>R^v_1,G_n\}\\
\end{align*}

Thus we have:

\begin{align}
\mc{E}^c_z(n_1)\subseteq & \left[ \bigcup_{n_0\le n \le n_1} \left(\{E_{n+1}>R^z_1-R^z_0 ,G_n\}\cup \{||\bar v_{n+1}||>R_1^v,G_n\}\right)\right]\\ 
&\ \ \ \cup \left[ \bigcup_{n\ge n_1+1}\{E^*_{n+1}>\epsilon,G_n\}\cup\{||v_{n+1}||>R^v_1,G_n\}\right]
\end{align}

\end{proof}


\subsection{Bounding the Fast Time Scale}
We now state a first Lemma that provides a high probability bound on $\bar v_n$, on the event $G_n$, where $G_n=\{ v_i \in B_{R^v_1}(0) \ \ i=n_0,...,n-1 \}\cap \{z_i \in B_{R_z}(z^*) \ \ i=n_0,...,n-1\}$ for $n_0$ to be defined.

\begin{lemma}

There exists positive constants $c,K_1$ such that:

\[ Pr(||\bar v_{n_1}||\ge \epsilon| G_{n_1})\le \begin{cases}2d^2exp(-\frac{c\epsilon^2}{d^3b_n} ) \ \ &: \epsilon \in \left(0,\frac{K_1 d \sqrt{d}}{\sigma_{max}^2}\right)\\
2d^2exp(-\frac{c\epsilon}{d \sqrt{d}b_n}) &: \text{otherwise}\end{cases} \]
\label{lemma:vconc}
\end{lemma}



\begin{proof}
We first note that $||B(z_n)||=1-b_n\sigma^2_{max}:=\delta_n$ for $b_n<1/\sigma^2_{max}$. Letting $R^v_0=||v_{n_0}||$, we first derive a bound for \eqref{term:t1v} on the event $G_n=\{ v_i \in B_{R^v_1}(0)\ \  and \ \ z_i \in B_{R_z}(z^*) \ \ i=n_0,...,n\}$: 

\[\left\Vert\prod_{i=n_0}^{n_0+n}B(z_i)\bar v_{n_0}\right\Vert \le   R^v_0 \prod_{i=n_0}^{n_0+n} \delta_i \]

We now bound $||\Delta_i||$. By definition:

\begin{align*}
||\Delta_i||&=||v^*_{i-1}-v^*_i||\\
&=||J^{-1}(z_{i-1})\omega(z_{i-1})-J^{-1}(z_{i})\omega(z_{i})||\\
&=\left(L_\omega+\frac{1}{L_J}\right)max\left(\sigma_{max},\frac{1}{\sigma_{min}}\right)||z_i-z_{i-1}||\\
\end{align*}

We now expand $z_{i+1}$, and get:

\begin{align*}
||z_{i+1}-z_{i}||&=a_{i}||h(z_i)-J^T(z_{i})\bar v_i+M^z_{i+1}||
\end{align*}

Since $h(z_i)=\omega(z_i)+J^{-1}(z_{i})\omega(z_{i})$,

\[ ||h(z_i)||\le L_f+\frac{L_f}{\sigma_{min}} :=L_h \]

Further, on $G_n$, $||\bar v_i||<R^v_1$. Therefore:

\[ ||J^T(z_i)\bar v_i||\le \sigma_{max}R^v_1 \]

Letting $L^*=\left(L_\omega+\frac{1}{L_J}\right)max\left(\sigma_{max},\frac{1}{\sigma_{min}}\right)$, we have:

\[||\Delta_i||\le a_{i-1}L^*(L_h+\sigma_{max}R^v_1)+a_{i-1}L^*||M^z_i||\]

We now rewrite the term in \eqref{term:t2v}. %Using the assumption that $||M_{n+1}^z||\le c_z(1+||z_n||)$: we get, that on $G_n$:

\[||\Delta_i||\le a_{i-1}L^*(L_h+\sigma_{max}R^v_1)+a_{i-1}L^*||M_{n+1}^z||\]

Letting, $L_\Delta=L^*(L_h+\sigma_{max}R^v_1)$:

\begin{align*} \left\Vert\sum_{i=n_0}^{n_1-1}\left(\prod_{j=i+1}^{n_1-1}B(z_j)\right)\Delta_{i+1}\right\Vert&\le \sum_{i=n_0}^{n_1-2} a_i(L_\Delta +L^*||M_{i+1}^z||) \left\Vert\left(\prod_{j=i+1}^{n_1-1}B(z_j)\right)\right\Vert\\
&\le L_\Delta \sum_{i=n_0}^{n_1-1} \frac{a_i}{b_{i+1}} \left\Vert\left(b_{i+1}\prod_{j=i+1}^{n_1-1}B(z_j)\right)\right\Vert\\
&\ \ \ \ \ +L^*\sum_{i=n_0}^{n_1-1} \frac{a_i}{b_{i}}||M_{i+1}^z|| \left\Vert\left(b_{i}\prod_{j=i+1}^{n_1-1}B(z_j)\right)\right\Vert\\
\end{align*}


We note that $\left\Vert\left(\prod_{j=i+1}^{n_1-1}B(z_j)\right)\right\Vert \le \prod_{j=i+1}^{n_1-1}\delta_j$. Using that fact that $b_{i+1}\prod_{j=i+1}^{n_1-1}\delta_j\le \frac{1}{\sigma^2_{max}}$, we finally get that:

\[\left\Vert\sum_{i=n_0}^{n_1-1}\left(\prod_{j=i+1}^{n_1-1}B(z_j)\right)\Delta_{i+1}\right\Vert\le \frac{L_\Delta}{\sigma^2_{max}} \sup_{i\in [n_0,n_1]} \frac{a_i}{b_{i+1}} + \frac{L^*}{\sigma^2_{max}}\sup_{n_0\le n\le n_1-1}\frac{a_n}{b_{n}} ||M_{n+1}^z||\]

Putting these together, and letting $\sum_{i=n_0}^{n_1-1}b_i\left(\prod_{j=i+1}^{n_1-1}B(z_j) \right)M^v_{i+1}:=S_v(n_0,n_1)$ we get that:
\begin{align*}
||\bar v_{n_1}||\le&  R^v_0 \prod_{i=n_0}^{n_0+n} \delta_i\\
&+\frac{L_\Delta}{\sigma^2_{max}} \sup_{i\in [n_0,n_1]} \frac{a_i}{b_{i+1}}\\
&+||S_v(n_0,n_1)||\\
&+ \frac{L^*}{\sigma^2_{max}}\sup_{n_0\le n\le n_1-1}\frac{a_n}{b_{n}} ||M_{n+1}^z||
\end{align*}

Now, since $\lim_{i\rar \infty} \frac{a_i}{b_{i+1}}=0$, and choosing $n_0$ large enough that $\sup_{i\in [n_0,\infty)} \frac{a_i}{b_{i+1}}\le \frac{\epsilon \sigma^2_{max} }{4L_\Delta}$, and $n_1$ large enough such that $\prod_{i=n_0}^{n_0+n} \delta_i \le \frac{\epsilon}{4R^v_0 }$ we get that, on $G_{n_1}$:

\begin{align*}
||\bar v_{n_1}||\le \frac{\epsilon}{2}+||S_v(n_0,n_1)||+\frac{L^*}{\sigma^2_{max}}\sup_{n_0\le n\le n_1-1}\frac{a_n}{b_{n}} ||M_{n+1}^z||\\
\end{align*}

Therefore:
\[\{ ||\bar v_{n_1}||>\epsilon, G_n \}\subseteq \left\{ ||S_v(n_0,n_1)|| >\frac{\epsilon}{4}, G_n\right\}\cup  \left\{ \sup_{n_0\le n\le n_1-1}\frac{a_n}{b_{n}} ||M_{n+1}^z||> \frac{\sigma^2_{max}\epsilon}{4L^*},G_n\right\}\]

We finish by finding a super-set of the second event on the left above:
 \[ \left\{ \sup_{n_0\le n\le n_1-1}\frac{a_n}{b_{n}} ||M_{n+1}^z||> \frac{\sigma^2_{max}\epsilon}{4L^*},G_n\right\}\subseteq\bigcup_{n=n_0}^{n_1-1}\left\{G_{n},\frac{a_n}{b_{n}} ||M_{n+1}^z||> \frac{\sigma^2_{max}\epsilon}{4L^*}\right\}\]

 Putting these together gives:

\begin{align*}
\{ ||\bar v_{n_1}||>\epsilon, G_n \}\subseteq& \left\{ ||S_v(n_0,n_1)|| >\frac{\epsilon}{4}, G_n\right\}\\
& \ \ \ \cup \bigcup_{n=n_0}^{n_1-1}\left\{G_{n},\frac{a_n}{b_{n}} ||M_{n+1}^z||> \frac{\sigma^2_{max}\epsilon}{4L^*}\right\}
\end{align*}


% Now, we bound $||S_v(n_0,n_1)||$ using \tc{red}{CITE BORKAR CONC INEQ}. Note that $S_v(n_0,n_1)$  is a martingale and that $||b_i\prod_{j=i+1}^{n_1-1}B(z_j)||\le b_i exp(-\sigma^2_{max} \sum_{j=i+1}^{n_1-1}b_j):=A_{i,n}$. Further note that $\mathbb{E}[exp(||M^v_{n+1}||)|G_n,\mc{F}_n]\le exp(c_1(1+R^v_0)):=K_1$, $\sum_{j=i}^{n} A_{j,n}\le \frac{1}{\sigma_{max}^2}$, and $\max_{n_0\le k\le n}A_{k,n}=b_n$. Since all the conditions are satisfied, we have that:

% \begin{align*}
% Pr(||S^v_v(n_0,n_1)||\ge \epsilon/4)\le \begin{cases}2d^2exp(-\frac{c\epsilon^2}{d^3b_n}) \ \ &: \epsilon \in \left(0,\frac{K_1 d \sqrt{d}}{\sigma_{max}^2}\right)\\
% 2d^2exp(-\frac{c\epsilon}{d \sqrt{d}b_n}) &: \text{otherwise}\end{cases} 
% \end{align*}

% We finish by bounding $\sup_{n_0\le n\le n_1+1}\frac{a_n}{b_{n}} ||M_{n+1}^z||$. By assumption, $Pr(||M_{n+1}^z||>\epsilon)<c_1exp(-c_2\epsilon)$. Thus:
% \begin{align*}
% Pr\left(\sup_{n_0\le n\le n_1-1}\frac{a_n}{b_{n}} ||M_{n+1}^z||>\epsilon\right)&\le 1-\sum_{i=n_0}^{n_1-1}Pr\left(\frac{a_n}{b_{n}} ||M_{n+1}^z||\le\epsilon\right)
% \end{align*}

% The desired result follows.
\end{proof}


We now bound the slow-varying process using Alekseev's formula, which allows us to treat the error from the fast-time scale and the noise as perturbations to the limiting ode, $\dot z=-h(z)$. To do so, 
We first derive a useful bound which will be useful in our further developments:

\begin{lemma}
There exists a positive constant $C_1$ depending on $\sigma_{max}, L_h,$ and $R_1^z$ such that:
\begin{align}
&\int_{t_k}^{t_{k+1}}e^{-\lambda(t_n-s)}||\bar z(s)-\bar z(t_k)||ds \le C_1 a_k^2e^{-\lambda(t_n-t_{k+1})}(1+||M_{k+1}^z||)
\end{align}
\label{lemma:genbnd}
\end{lemma}

\begin{proof}

\begin{align*}
||\bz(s)-\bz(t_k)||&=\frac{s-t_k}{a_k}||\bz(t_{k+1})-\bz(t_k)||\\
&\le(s-t_k)||h(\bz(t_k))+J^T(\bz(t_k))\bar v_k+M_{k+1}^z||\\
&\le(s-t_k)(L_h+\sigma_{max}||\bar v_k||+||M_{k+1}^z||)\\
\end{align*}

Since $\int_{t_k}^{t_{k+1}}(s-t)e^{-\lambda(t_n-s)}ds\le a_k^2 e^{-\lambda(t_n-t_{k+1})}$:

\begin{align*}
\int_{t_k}^{t_{k+1}}&e^{-\lambda(t_n-s)}||\bar z(s)-\bar z(t_k)||ds\\
&\le a_k^2 e^{-\lambda(t_n-t_{k+1})} (L_h+\sigma_{max}||\bar v_k||+||M_k^z||)\\
\end{align*}
Now, remarking that on $G_n$, $||\bar v_k||\le R_v$ our result follows.
\end{proof}

We now derive a bound on $||W_n||$ using Lemma~\ref{lemma:genbnd}.

\begin{lemma}
There exists a positive constant $C_2$ depending on $C_1,K_2,L_h, \lambda$ such that:
\begin{align}
||W_n||\le C_2\left(\sup_{n_0\le k \le n-1}a_k+\sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||\right)
\end{align}
\label{lemma:Wbnd}
\end{lemma}

\begin{proof}
\begin{align*}
||W_n||&\le \sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}||\Phi(t_n,s,\bz(s))||h(\bz(t_k))-h(\bz(s))||ds\\
&\le L_h K_2 \sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}} e^{-\lambda(t_n-s)}||\bz(t_k)-\bz(s)||ds\\
&\le L_h K_2 C_1 \sum_{k=n_0}^{n-1}a_k^2 (1+||M_{k+1}^z||)e^{-\lambda(t_n-t_{k+1})}\\
&\le L_h K_2 C_1 \left(\sup_{n_0\le k \le n-1}a_k+\sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||\right)\sum_{k=n_0}^{n-1}a_ke^{-\lambda(t_n-t_{k+1})}\\
\end{align*}

Now, using the fact that $\sum_{k=n_0}^{n-1}a_ke^{-\lambda(t_n-t_{k+1})}\le \frac{1}{\lambda}$, the desired result follows.
\end{proof}

We now derive a bound on $||\tilde S^z_n-S^z_n||$ and $||\tilde V_n-V_n||$. 

\begin{lemma}
There exists a positive constant $C_3$ depending on $C_1,K_3,\lambda,R^z_1$ such that, on $G_n$:
\begin{align}
||\tilde S^z_n-S^z_n||&\le C_3 \left(\sup_{n_0\le k \le n-1}a_k+\sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||^2\right)\\
\end{align}
\label{lemma:Sbnd}
\end{lemma}


\begin{proof}
\begin{align*}
||\tilde S^z_n-S^z_n||&\le\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}||\Phi(t_n,s,\bz(s))-\Phi(t_n,s,\bz(t_{k})||ds||M_{k+1}^z||  \\
&\le K_3 C_1 \sum_{k=n_0}^{n-1}a^2_k(1+||M_{k+1}^z||)||M_{k+1}^z||e^{-\lambda(t_n-t_{k+1})}\\
&\le K_3 C_1 \left(\sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||+\sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||^2\right)\sum_{k=n_0}^{n-1}a_ke^{-\lambda(t_n-t_{k+1})}
\end{align*}

Using the fact that $||x|| \le 1+||x||^2$, finishes the proof.
\end{proof}


\begin{lemma}
There exists a positive constant $C_4$ depending on $C_1,K_3,\lambda,R^v_1$ such that, on $G_n$:
\begin{align}
||\tilde V_n-V_n||&\le C_4 \left(\sup_{n_0\le k \le n-1}a_k+\sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||\right)
\end{align}
\label{lemma:Vbnd}
\end{lemma}

\begin{proof}
\begin{align*}
||\tilde V_n-V_n||&\le\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}||\Phi(t_n,s,\bz(s))-\Phi(t_n,s,\bz(t_{k})||ds||v_{k+1}||  \\
&\le K_3 C_1 R^v_1 \sum_{k=n_0}^{n-1}a^2_kC_1\left(1+||M^z_{k+1}||\right)e^{-\lambda(t_n-t_{k+1})}\\
&\le K_3 C_1 R^v_1 \left(\sup_{n_0\le k \le n-1}a_k+\sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||\right)\sum_{k=n_0}^{n-1}a_ke^{-\lambda(t_n-t_{k+1})}
\end{align*}

Where the second inequality follows by using the fact that, on $G_n$, $||\bar v_k||\le R_1^v$, and then using \tc{red}{BORthm3} and then Lemma~\ref{lemma:genbnd}. Now using the fact that $\sum_{k=n_0}^{n-1}a_ke^{-\lambda(t_n-t_{k+1})}\le \frac{1}{\lambda}$, the desired result follows.
\end{proof}

We now find an intermediate bound on $V_n$.

\begin{lemma}
There exists a positive constant $C_5$ depending on $\lambda$ such that, on $G_n$:
\begin{align}
||V_n|| \le C_5\sup_{n_0\le k \le n}||\bar v_k||
\end{align}
\label{lemma:Vbnd2}
\end{lemma}

\begin{proof}
\begin{align*}
||V_n|| &\le \sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}||\Phi(t_n,s,\bar z(t_k))||ds ||\bar v_{t_k}||\\
&\le \left(\sup_{n_0\le k \le n-1}||\bar v_{t_k}||\right) \sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}||\Phi(t_n,s,\bar z(t_k))||ds
\end{align*}

Now, looking at $\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}||\Phi(t_n,s,\bar z(t_k))||ds$:

\begin{align*}
\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}||\Phi(t,s,\bar z(t_k))||ds&\le \frac{K_2 }{\lambda}\sum_{k=n_0}^{n-1} e^{-\lambda(t_n-t_{k})}-e^{-\lambda(t_n-t_{k-1})}\\
&\le \frac{K_2 }{\lambda}e^{-\lambda(t_n-t_{n-1})}=\frac{K_2 }{\lambda}e^{-a_{n-1}\lambda }\le \frac{K_2 }{\lambda}
\end{align*}

Which completes the proof.

\end{proof}


With Lemmas \ref{lemma:Wbnd}-\ref{lemma:Vbnd2} we now construct a bound on $||\bz(t_n)-z(t_n,t_{n_0},\bar z(t_{n_0}))||$ on $G_n$:


\begin{lemma}
\label{lemma:z1}
Let $n\ge n_0$ be arbitrary. Further, let $C_6=max(C_2,C_3,C_4,C_5)$. Then on $G_n$:

\begin{align*}
||\bz(t_n)-z(t_n,t_{n_0},\bar z(t_{n_0}))||&\le C_6\left(\sup_{n_0\le k \le n-1}a_k+ \sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||^2+\sup_{n_0\le k \le n}||\bar v_k||\right)+||S_n^z||
\end{align*}
\end{lemma}

\begin{proof}
\begin{align*}
||\bz(t_n)-z(t_n,t_{n_0},\bar z(t_{n_0}))||\le& C_2\left(\sup_{n_0\le k \le n-1}a_k+\sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||\right)\\
&\ \ +C_3 \left(\sup_{n_0\le k \le n-1}a_k+\sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||^2\right)\\
&\ \ +C_4 \left(\sup_{n_0\le k \le n-1}a_k+\sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||\right)\\
&\ \ +C_5\sup_{n_0\le k \le n-1}||\bar v_k||+||S_n^z||
\end{align*}

Letting $C_6=max(C_2,C_3,C_4,C_5)$, and using again using $||x|| \le 1+||x||^2$, finishes the proof.
\end{proof}

\[||\bz(t_n)-z(t_n,t_{n_0},\bar z(t_{n_0}))||\le C_6\left(\sup_{n_0\le k \le n-1}a_k+\sup_{n_0\le k \le n-1}a_k||M^z_{k+1}||^2+\sup_{n_0\le k \le n}||\bar v_k||\right)+||S_n^z||\]

To be able to construct a bound on the event $E_{n+1}$ we also have to bound, $||\bz(t_{n+1})-z(t_{n+1},t_{n_0},\bar z(t_{n_0}))||$ on $G_n$. 



\begin{lemma}
\label{lemma:z2}
Let $n\ge n_0$ be arbitrary. Then there exists a positive constant $C_7$ depending on $C_6, L_h, R^z_1, \sigma_{max}, and R^v_1$ such that, on $G_n$:
\[ ||\bz(t_{n+1})-z(t_{n+1},t_{n_0},\bar z(t_{n_0}))||\le C_7\left(\sup_{n_0\le k \le n}a_k+\sup_{n_0\le k \le n}a_k||M^z_{k+1}||^2+\sup_{n_0\le k \le n}||\bar v_k||+||S_n^z||\right)\]
\end{lemma}

\begin{proof}
Note that:
\[ z(t_{n+1},t_{n_0},\bar z(t_{n_0}))=z(t_n,t_{n_0},\bar z(t_{n_0}))+\int_{t_n}^{t_{n+1}}h(z(s,t_{n_0},\bar z(t_{n_0})))ds \]

Thus, it follows that:

\begin{align*}
||\bz(t_{n+1})-z(t_{n+1},t_{n_0},\bar z(t_{n_0}))||&\le ||\bz(t_n)-z(t_n,t_{n_0},\bar z(t_{n_0}))||+a_n||M^z_{n+1}||+a_n||J^T(\bz(t_n))\bar v_n||\\
& \ \ +\int_{t_n}^{t_{n+1}}||h(\bz(t_n))-h(z(s,t_{n_0},\bar z(t_{n_0})))||ds
\end{align*}

Now since $h$ is $L_h$-Lipschitz on $G_n$, and for all $s\ge t_{n_0}$, $z(s,t_{n_0},\bar z(t_{n_0})) \in B_{R^z_1}(z^*)$ by construction, then:

\[ \int_{t_n}^{t_{n+1}}||h(\bz(t_n))-h(z(s,t_{n_0},\bar z(t_{n_0})))||ds\le 2L_h R^z_1a_n \]

Similarly, on $G_n$, we know that $||\bar v_n||\le R^v_1$. Therefore:

\begin{align*}
||\bz(t_{n+1})-z(t_{n+1},t_{n_0},\bar z(t_{n_0}))||&\le ||\bz(t_n)-z(t_n,t_{n_0},\bar z(t_{n_0}))||\\
&\ \ \ +a_n||M^z_{n+1}||+a_n\sigma_{max}R^v_1+2L_h R^z_1a_n
\end{align*} 

Now using our bound on $||\bz(t_n)-z(t_n,t_{n_0},\bar z(t_{n_0}))||$ completes the proof.

\end{proof}

We are now finally ready to bound $E_{n+1}$ on $G_n$.

\begin{lemma}
\label{lemma:En}
Let $n\ge n_0$ be arbitrary. There exists a positive constant $K$ depending only on $C_7, L_h, R^z_1$ such that, on $G_n$:

\[ E_{n+1}\le K\left(\sup_{n_0\le k \le n}a_k+\sup_{n_0\le k \le n}a_k||M^z_{k+1}||^2+\sup_{n_0\le k \le n}||\bar v_k||+||S_n^z||\right)\]
\end{lemma}


\begin{proof}
For $t \in [t_n,t_{n=1}]$, $\bz(t)$ is a convex combination of $\bz(t_n)$ and $\bz(t_{n+1})$. Therefore for each $t \in [t_n,t_{n=1}]$, there exists $\gamma \in [0,1]$ such that:
\[ \bz(t)=(1-\gamma)\bz(t_n)+\gamma \bz(t_{n+1})\]
Therefore:

\[ || \bz(t)-z(t,t_{n_0},\bz(t_{n_0}))||\le (1-\gamma)||\bz(t_n)-z(t,t_{n_0},\bar z(t_{n_0}))||+\gamma||\bz(t_{n+1})-z(t,t_{n_0},\bar z(t_{n_0}))||\]

Now note that:
\[ z(t_{n+1},t_{n_0},\bar z(t_{n_0}))=z(t,t_{n_0},\bar z(t_{n_0}))+\int_{t}^{t_{n+1}}h(z(s,t_{n_0},\bar z(t_{n_0})))ds\]
\[ z(t,t_{n_0},\bar z(t_{n_0}))=z(t_n,t_{n_0},\bar z(t_{n_0}))+\int_{t_n}^{t}h(z(s,t_{n_0},\bar z(t_{n_0})))ds\]

Using the above two inequalities gives us:

\begin{align*}
|| \bz(t)-z(t,t_{n_0},\bz(t_{n_0}))||&\le (1-\gamma)||\bz(t_n)-z(t_n,t_{n_0},\bar z(t_{n_0}))||\\
&\ \ \ +\gamma||\bz(t_{n+1})-z(t_{n+1},t_{n_0},\bar z(t_{n_0}))||\\
&\ \ \ +\int_{t_n}^{t_{n+1}}||h(z(s,t_{n_0},\bar z(t_{n_0})))||ds
\end{align*}

Now, since $\int_{t_n}^{t_{n+1}}||h(z(s,t_{n_0},\bar z(t_{n_0})))||=\int_{t_n}^{t_{n+1}}||h(z^*)-h(z(s,t_{n_0},\bar z(t_{n_0})))||$, and $z(s,t_{n_0},\bar z(t_{n_0})) \in B_{R^z_1}(z^*)$ for all $s\ge t_{n_0}$ gives: $\int_{t_n}^{t_{n+1}}||h(z(s,t_{n_0},\bar z(t_{n_0})))||ds \le a_n L_h R^z_1$.

Putting together Lemma \ref{lemma:z1} and Lemma \ref{lemma:z2}, gives us our result.
\end{proof}


Similarly, we can bound $E^*_{n+1}$ on $G_n$.

\begin{lemma}
\label{lemma:En}
Let $n\ge n_0$ be arbitrary. There exists a positive constant $K$ depending only on $C_8, K_1,R^z_0$ such that, on $G_n$:

\[ E^*_{n+1}\le K\left(\sup_{n_0\le k \le n}a_k+\sup_{n_0\le k \le n}a_k||M^z_{k+1}||^2+\sup_{n_0\le k \le n}||\bar v_k||+||S_n^z|| + e^{-\lambda(t_n-t_{n_0})}\right)\]
\end{lemma}

\begin{proof}
\begin{align*}
||\bz(t)-z^*||\le ||\bz(t)-z(t,t_{n_0},\bz(t_{n_0}))||+||z(t,t_{n_0},\bz(t_{n_0}))-z^*||
\end{align*}

Now, on $G_n$ using \tc{red}{CITE BORKAR}:
\begin{align*}
 ||z(t,t_{n_0},\bz(t_{n_0}))-z^*||\le K_1 || \bz(t_{n_0})-z^*||e^{-\lambda(t_n-t_{n_0})} \le K_1 R^z_0 e^{-\lambda(t_n-t_{n_0})}
 \end{align*}

 Substituting in above, and using Lemma \ref{lemma:En} gives the desire result.

\end{proof}

Now let us analyze the events that we would like to bound. Choose $n_1$ large enough such that $e^{-\lambda(t_n-t_{n_0})}<\frac{\epsilon}{5K}$ and $n_0$ large enough such that $\sup_{n_0\le k \le n}a_k \le \frac{\epsilon}{5K}$. Then:
\begin{align*}
\{E^*_{n+1}>\epsilon,G_n\}\subseteq& \left\{ \sup_{n_0\le k \le n}a_k||M^z_{k+1}||^2 >\frac{\epsilon}{5K}  , G_n\right\}\\
&\ \ \ \cup \left\{ ||S_n^z|| >\frac{\epsilon}{5K}, G_n \right\}\\
&\ \ \ \cup \left\{ \sup_{n_0\le k \le n}||\bar v_k|| >\frac{\epsilon}{5K} , G_n \right\}
\end{align*}

We find a superset of the first event by noting that, for $k<n$, $G_n \subset G_k $:
\[\left\{ \sup_{n_0\le k \le n}a_k||M^z_{k+1}||^2 >\frac{\epsilon}{5K}  , G_n\right\}\subseteq \bigcup_{n_0 \le k \le n} \left\{ a_k||M^z_{k+1}||^2 >\frac{\epsilon}{5K}, G_k \right\}\]


Similarly for the last event:
\[\left\{ \sup_{n_0\le k \le n}||\bar v_k|| >\frac{\epsilon}{5K}, G_n \right\}\subseteq \bigcup_{n_0 \le k \le n} \left\{ ||\bar v_k|| >\frac{\epsilon}{5K}, G_k \right\}\]

Thus: 

\begin{align*}
\{E^*_{n+1}>\epsilon,G_n\}\subseteq& \left[  \bigcup_{n_0 \le k \le n} \left\{ a_k||M^z_{k+1}||^2 >\frac{\epsilon}{5K}, G_k \right\}\right]\\
&\ \ \ \cup \left\{ ||S_n^z|| >\frac{\epsilon}{5K}, G_n \right\}\\
&\ \ \ \cup \left[ \bigcup_{n_0 \le k \le n} \left\{ ||\bar v_k|| >\frac{\epsilon}{5K}, G_k \right\}\right]
\end{align*}

Now, let $R^z_1-R^z_0=R_z$. Suppose that $R_z>\frac{\epsilon}{5}$. Choose $n_0$ large enough such that $\sup_{n_0\le k \le n}a_k \le \frac{R_z}{4K}$.  We now find a superset of the event $\{E_{n+1}>R_z,G_n\}$.

\begin{align*}
\{E_{n+1}>R_z,G_n\}&\subseteq \left[  \bigcup_{n_0 \le k \le n} \left\{ a_k||M^z_{k+1}||^2 >\frac{\epsilon}{5K}, G_k \right\}\right]\\
&\ \ \ \cup \left\{ ||S_n^z|| >\frac{\epsilon}{5K}, G_n \right\}\\
&\ \ \ \cup \left[ \bigcup_{n_0 \le k \le n} \left\{ ||\bar v_k|| >\frac{\epsilon}{5K}, G_k \right\}\right]
\end{align*}

Now putting this all together:

\begin{align}
\mc{E}^c_z(n_1)\subseteq& \bigcup_{k\ge n_0} \left\{ a_k||M^z_{k+1}||^2 >\frac{\epsilon}{5K}, G_k \right\}\\
& \ \ \ \cup  \bigcup_{k\ge n_0}  \left\{ ||\bar v_k|| >\frac{\epsilon}{5K}, G_k \right\}\\
& \ \ \ \cup  \bigcup_{k\ge n_0}  \left\{ ||S_k^z|| >\frac{\epsilon}{5K}, G_k \right\}\\
& \ \ \ \cup  \bigcup_{k\ge n_0}  \left\{ ||\bar v_k|| >R^v_1, G_k \right\}\\
\end{align}

Now, since $\frac{\epsilon}{5K}<R^v_1$, this can be simplified to:

\begin{align}
\mc{E}^c_z(n_1)\subseteq& \bigcup_{k\ge n_0} \left\{ a_k||M^z_{k+1}||^2 >\frac{\epsilon}{5K}, G_k \right\}\\
& \ \ \ \cup  \bigcup_{k\ge n_0}  \left\{ ||S_k^z|| >\frac{\epsilon}{5K}, G_k \right\}\\
& \ \ \ \cup  \bigcup_{k\ge n_0}  \left\{ ||\bar v_k|| >\frac{\epsilon}{5K}, G_k \right\}\\
\end{align}

Using our earlier result gives:


\begin{align}
\mc{E}^c_z(n_1)\subseteq& \bigcup_{k\ge n_0} \left\{ a_k||M^z_{k+1}||^2 >\frac{\epsilon}{5K}, G_k \right\}\\
& \ \ \ \cup  \bigcup_{k\ge n_0}  \left\{ ||S_k^z|| >\frac{\epsilon}{5K}, G_k \right\}\\
& \ \ \ \cup  \bigcup_{k\ge n_0} \left\{ ||S_v(n_0,k)|| >\frac{\epsilon}{20K}, G_k\right\}\\
& \ \ \ \cup \bigcup_{k\ge n_0}\left\{\frac{a_k}{b_{k}} ||M_{k+1}^z||> \frac{\sigma^2_{max}\epsilon}{20L^*K},G_k\right\}
\end{align}

Using all of the bounds, and defining $\eta_n:=\frac{a_n}{b_n}$ this gives us:

\begin{align*}
Pr(\mc{E}^c_z(n_1)) \le & c_1\sum_{n=n_0}^\infty exp\left(-c_2\frac{\sqrt{\epsilon}}{\sqrt{a_n}}\right)\\
&\ \ \ +c_1\sum_{n=n_0}^\infty exp\left(-c_5\frac{\epsilon^2}{\eta_n}\right)\\
&\ \ \ +2d^2\sum_{n=n_0}^\infty exp\left(-c_3\frac{\epsilon^2}{a_n}\right)\\
&\ \ \ +2d^2\sum_{n=n_0}^\infty exp\left(-c_4\frac{\epsilon^2}{b_n}\right)\\
\end{align*}

Now, note that $a_n$, $b_n$, $\eta_n$ $\rar0$, and thus all of these sums are finite. Therefore:

\begin{align*}
Pr(\mc{E}_z(n_1)) \le & 1- c_1\sum_{n=n_0}^\infty exp\left(-c_2\frac{\sqrt{\epsilon}}{\sqrt{a_n}}\right)\\
&\ \ \ -c_1\sum_{n=n_0}^\infty exp\left(-c_5\frac{\epsilon^2}{\eta_n}\right)\\
&\ \ \ -2d^2\sum_{n=n_0}^\infty exp\left(-c_3\frac{\epsilon^2}{a_n}\right)\\
&\ \ \ -2d^2\sum_{n=n_0}^\infty exp\left(-c_4\frac{\epsilon^2}{b_n}\right)\\
\end{align*}

Now, let us assume $a_n=1/(1+n)^\alpha$, and $b_n=1/(1+n)^\beta$, where $0<\beta<\alpha<1$. Choosing $\beta=\alpha/2$ gives us convergence on the same order as the original process (when using the Borkar Result).

\begin{align*}
Pr(\mc{E}_z(n_1)) \le & 1- O\left(n_0^{1-\alpha/2}e^{-Cn_0^{\alpha/2}}\right)
\end{align*}









==> thm_copy.tex <==
% !TEX root = TTS_JMLR18.tex


The event we would like to bound is: $\{||z_n-z^*||<\epsilon \forall n\ge n_1\}$ on the event $\{||z_{n_0}-z^*||\le R_0^z\}$. where $n_1>n_0$. W will construct an upper bound on the complement of this event using the bounds we have just constructed and the martingale concentration inequality used in Lemma \ref{lemma:vconc}.

\begin{lemma}
\label{lemma:event}
\[\mc{E}^c_z(n_1)\subseteq \left[ \bigcup_{n_0\le n \le n_1} \left(\{E_{n+1}>R^z_1-R^z_0 ,G_n\}\cup \{||\bar v_{n+1}||>R^v,G_n\}\right)\right]\cup \left[ \bigcup_{n\ge n_1+1}\{E^*_{n+1}>\epsilon_1,||v_{n+1}||>R^v,G_n\}\right]\]
\end{lemma}

\begin{proof}
Define:
\[\mc{E}_z(n_1):=\{||\bar z(t)-z^*||<\epsilon_1 \ \ \forall \  t\ge t_{n_1+1}\}\cap \{||\bar v_n||<R^v \ \ \forall \  n\ge n_1+1\} \]
\[ B_{R^z_1}(z^*):=\{z: ||z-z^*|| \le R^z_1\}\]
\[ B_{R^v}(0):=\{v: ||v|| \le R^v\}\]
\[ E_{n+1}:=\sup_{t \in [t_n, t_{n+1}]} || \bar z(t)-z(t,t_{n_0},\bar z(t_{n_0}))||\]
\[ E^*_{n+1}:=\sup_{t \in [t_n, t_{n+1}]} || \bar z(t)-z^*||\]
\[ G^z_n:=\{\bz(t) \in B_{R^z}(z^*) \ \forall t \in [t_{n_0},t_n]\}\]
\[ G^v_n:=\{\bar v_k \in B_{R^v}(0) ; k=n_0,...,n\}\]
\[ G^{gap}_n:=\{\sup_{n_0\le k \le n } E_{k+1} >R^z_1-R^z_0\}\]
\[ G_n=G^z_n \cap G^v_n\]
\[ D_n=G^{gap}_n \cap G^v_n\]


We would like to find a superset of $\mc{E}^c_z(n_1)$ where $n_1=n_0+N$. 

%First, note that $\mc{E}_z(n_1)=\bigcap_{n=n_1+1}^{\infty} \{ E^*_{n+1} \le \epsilon \}$. Therefore $\mc{E}^c_z(n_1)=\bigcup_{n=n_1+1}^{\infty} \{ E^*_{n+1} > \epsilon \}$. 

%Now, $\bigcup_{n=n_1+1}^{\infty} \{ E^*_{n+1} > \epsilon \} \subseteq G_{n_1}^c \cup \bigcup_{n=n_1+1}^{\infty} \{ E^*_{n+1} > \epsilon \}$


\[ \mc{E}^c_z(n_1)= (\mc{E}^c_z(n_1)\cap D_{n_1}^c)\cup(\mc{E}^c_z(n_1)\cap D_{n_1}) \subseteq D_{n_1}^c\cup(\mc{E}^c_z(n_1)\cap D_{n_1})\]

We first analyze $D_{n_1}^c$:
\begin{align*}
D_{n_1}^c&=(G^{gap}_{n_1})^c \cup (G^v_{n_1})^c\\
&=\{\sup_{n_0\le n \le n_1 }E_{n+1}>R^z_1-R^z_0\}\cup \{\sup_{n_0\le k\le n_1+1}||\bar v_k||>R^v\}\\
&=\left[(G^{gap}_{n_1})^c \cup (G^v_{n_1})^c\right] \cup \left[\left(G^{gap}_{n_1} \cap G^v_{n_1} \right) \cap \left(\{E_{n_1+1}>R^z_1-R^z_0\}\cup \{||\bar v_{n_1+1}||>R^v\}\right)\right]
\end{align*}

Doing this recursively, we get:

\begin{align*}
D_{n_1}^c&=\bigcup_{n_0\le n \le n_1}\left(G^{gap}_{n} \cap G^v_{n} \right) \cap \left(\{E_{n+1}>R^z_1-R^z_0\}\cup \{||\bar v_{n+1}||>R^v\}\right)
\end{align*}

Using the fact that $G^{gap}_n\subseteq G^z_n$: lets us write this as:

\begin{align*}
D_{n_1}^c&\subseteq\bigcup_{n_0\le n \le n_1}\left(G^{z}_{n} \cap G^v_{n} \right) \cap \left(\{E_{n+1}>R^z_1-R^z_0\}\cup \{||\bar v_{n+1}||>R^v\}\right)\\
&=\bigcup_{n_0\le n \le n_1} \left(\{E_{n+1}>R^z_1-R^z_0 ,G_n\}\cup \{||\bar v_{n+1}||>R^v,G_n\}\right)
\end{align*}

Now we analyze $(\mc{E}^c_z(n_1)\cap D_{n_1})$. Since $D_{n_1}\subseteq G_{n_1}$, we can expand this, and write:

\[ \mc{E}^c_z(n_1)\cap D_{n_1}\subseteq \mc{E}^c_z(n_1) \cap G_{n_1} = \bigcup_{n\ge n_1+1}\{E^*_{n+1}>\epsilon_1,||v_{n+1}||>\epsilon_2,G_n\}\]

Thus we have:

\[\mc{E}^c_z(n_1)\subseteq \left[ \bigcup_{n_0\le n \le n_1} \left(\{E_{n+1}>R^z_1-R^z_0 ,G_n\}\cup \{||\bar v_{n+1}||>R^v,G_n\}\right)\right]\cup \left[ \bigcup_{n\ge n_1+1}\{E^*_{n+1}>\epsilon_1,||v_{n+1}||>R^v,G_n\}\right]\]

\end{proof}

First, let $z^*$ be a LASE, of the desired dynamics $h$. By a converse Lyapunov Theorem \tc{red}{CITE CONVERSE LYAP} there exists a Lyapunov function $V$ such that $V(z^*)=0$, $V(z)>0$, $\nabla V(z)\dot h(z)<0$ for all $z \in U$, for $U\subset \X$. Let $R_z$ be the radius of the largest ball, centered at $z^*$ such that $B_{R_z}(z^*) \subset U$. We note that $Dh(z^*)$ has strictly positive eigenvalues from \tc{red}{CITE First thm}. Let $\lambda_n=Re(\lambda_{min}(Dh(z^*)))$. Now since $Dh(z^*)$ is symmetric, for all $\kappa \in (0,1)$, and defining $\lambda'=\kappa \lambda_n$, we know that $||exp(-Dh(z^*))||\le exp(-\lambda')$. 

We begin by stating our assumptions on the function, the estimator, and the step-sizes. We remark that these assumptions are more relaxed than what has been considered before in the literature on two-time scale processes, and are most similar to the conditions assumed for single time-scale processes analyzed in \tc{red}{CITE BORKAR ALEKSEEV}. We first make some assumptions on the function $f$.

\begin{assumption}{Assumptions on $f$:}
We assume that $f:\mb{R}^d\rar\mb{R} \in C^n$ for $n\ge2$. Then, since $B_{R_z}(z^*)$ is compact, both $\omega$ and $J$ must satisfy:
\begin{itemize}
	\item $f$ is $L_f$-Lipschitz continuous on $B_{R_z}(z^*)$.
	\item $\omega:\mb{R}^d\rar \mb{R}^d$ is $L_\omega$-Lipschitz continuous on $B_{R_z}(z^*)$.
	\item $J:\mb{R}^d \rar \mb{R}^{d\times d} $ is $L_J$-Lipschitz continuous on $B_{R_z}(z^*)$.
\end{itemize}
We further assume that $||J(z)||>\sigma_{min}>0 \ \ \forall \ \  z \in B_{R_z}(z^*)$ and define $\sigma_{max}=\max_{z \in B_{R_z}(z^*)} ||J(z)||$.
\label{ass:f}
\end{assumption}

We now state our assumptions on the sequence of step-sizes $a_n$ and $b_n$. We remark that we do not require either sequence to be square-summable.
\begin{assumption}{Assumptions on the step-sizes:}
We assume that $f \in C^n$ for $n\ge2$. Then, since $B_{R_z}(z^*)$ is compact, both $\omega$ and $J$ must satisfy:
\begin{itemize}
	\item $\lim_{n\rar \infty} a_n=0$, and $\lim_{n\rar \infty} b_n=0$.
	\item $\sum_{i=1}^\infty a_i=\infty$, and  $\sum_{i=1}^\infty a_i=\infty$.
	\item $\sup_{n\ge1} a_i \le 1$, and $\sup_{n\ge1} b_n \le 1$.
\end{itemize}
Finally we assume that the sequence $a_n$ decreases faster than $b_n$:  $\lim_{n \rar \infty} \frac{a_n}{b_n}=0$.
\label{ass:ss}
\end{assumption}

Finally we make further assumptions on the noise processes $M^z_n$, and  $M^v_n$. 

\begin{assumption}{Assumptions on the noise:}
We first define the filtration $\mc{F}_n$, $\mc{F}_n=\sigma(z_0,v_0,M^v_1,M^z_1,...,M^z_n,M^v_n)$ for $n\ge$. Given $\mc{F}_n$, we assume that:
\begin{itemize}
	\item $M_{n+1}^v$ and $M_{n+1}^z$ are conditionally independent given $\mc{F}_{n}$ for $n\ge0$.
	\item $\mb{E}[M_{n+1}^v|\mc{F}_n]=0$ and $\mb{E}[M_{n+1}^z|\mc{F}_n]=0$ for $n\ge0$.
	%\item $Pr(M_{n+1}^z>u|\mc{F}_n)\le c_1 exp(-c_2u)$ and $Pr(M_{n+1}^v>u|\mc{F}_n)\le c_3 exp(-c_4u)$ for $c_1,c_2,c_3,c_4>0$ and $u\ge \bar u>0$ for $\bar u$ sufficiently large.
	\item $||M_{n+1}^z||\le c_z(1+||z_n||)$ and $||M_{n+1}^v||\le c_v(1+||z_n||)$ almost surely.
\end{itemize}
\label{ass:noise}
\end{assumption}

We note that, in the last assumption the dependence is solely on $z_n$ due to the fact that the randomness in the process comes only from $\omega$ and $J$ which depend only on the current value of $z_n$. 

\begin{theorem}
Let R be the radius of the largest ball, centered at $z^*$, that fits in $dom(V)$, Let $R>R_1^z>R_0^z>0$. Further pick an $\epsilon$ such that $0<\epsilon<R_0^z$. Finally let $n_0=N_0(a_n,b_n,\epsilon_1,R_1^z)$, and $n_1=N_1(n_0,a_n,b_n,\epsilon_1,R_1^z)$. Then when $||z_{n_0}-z^*||\le R_0^z$ then:
\begin{align*} 
&Pr(||z_{n}-z^*||\le \epsilon,\ \ \forall n\ge n_1)\ge \\
 &\ \ \ \ \ \ \ 1-2d^2\sum_{n\ge n_0}\left[ exp\left[\frac{-C_1\sqrt{\epsilon}}{\sqrt{a_n}}\right]+exp\left[\frac{-C_2\epsilon}{a_n}\right]+exp\left[\frac{-C_3\epsilon}{b_n}\right] \right] 
\end{align*}
Where $C_1,C_2,C_3>0$ are constants depending on the parameters in the assumptions.
\label{thm:concbnd}
\end{theorem}

Before proving Theorem~\ref{thm:concbnd} we first derive a concentration bound for the fast-time scale $v_n$. To simplify our analysis, we first rewrite the fast time scale.  Let $\bar v_n=v_n-v^*_n$. Letting, $A_(z_n)=J^T(z_n)J(z_n)$, and $\Delta_{n+1}=v^*_n-v^*_{n+1}$, the update equation for $\bar v_n$ is given by:

\[ \bar v_{n+1}=\bar v_{n}-b_n[A(z_n)\bar v_n+M^v_{n+1}]+\Delta_{n+1}\]

Letting $B(z_n)=I-b_nA(z_n)$, this further simplifies to:

\[ \bar v_{n+1}=B(z_n)\bar v_n-b_n M^v_{n+1}+\Delta_{n+1}\]

The slow time-scale, as a function of $\bar v_n$ is given by:

\[z_{n+1}=z_n-a_n(h(z_n)-J^T(z_n)\bar v_n+M^z_n)\]

Letting $n_1=n_0+n+1$ we can now write:

\begin{align}
\bar v_{n_1}=&\prod_{i=n_0}^{n_0+n}B(z_i)\bar v_{n_0} \label{term:t1v}\\
&-\sum_{i=n_0}^{n_1-1}b_i\left(\prod_{j=i+1}^{n_1-1}B(z_j) \right)M^v_{i+1}\label{term:t2v}\\
&+\sum_{i=n_0}^{n_1-2}\left(\prod_{j=i+1}^{n_1-1}B(z_j)\right)\Delta_{i+1}\label{term:t3v}\\
&+\Delta_{n+1}\label{term:t4v}
\end{align}



We now state a first Lemma that provides a high probability bound on $\bar v_n$, on the event $G_n$, where $G_n=\{ v_i \in B_{R^v_1}(0) \ \ i=n_0,...,n-1 \}\cap \{z_i \in B_{R_z}(z^*) \ \ i=n_0,...,n-1\}$ for $n_0$ to be defined.

\begin{lemma}

There exists positive constants $c,K_1$ such that:

\[ Pr(||\bar v_{n_1}||\ge \epsilon| G_{n_1})\le \begin{cases}2d^2exp(-\frac{c\epsilon^2}{d^3b_n} ) \ \ &: \epsilon \in \left(0,\frac{K_1 d \sqrt{d}}{\sigma_{max}^2}\right)\\
2d^2exp(-\frac{c\epsilon}{d \sqrt{d}b_n}) &: \text{otherwise}\end{cases} \]
\label{lemma:vconc}
\end{lemma}



\begin{proof}
We first note that $||B(z_n)||=1-b_n\sigma^2_{max}:=\delta_n$ for $b_n<1/\sigma^2_{max}$. Letting $R^v_0=||v_{n_0}||$, we first derive a bound for \eqref{term:t1v} on the event $G_n=\{ v_i \in B_{R^v_1}(0)\ \  and \ \ z_i \in B_{R_z}(z^*) \ \ i=n_0,...,n\}$: 

\[\left\Vert\prod_{i=n_0}^{n_0+n}B(z_i)\bar v_{n_0}\right\Vert \le   R^v_0 \prod_{i=n_0}^{n_0+n} \delta_i \]

We now bound $||\Delta_i||$. By definition:

\begin{align*}
||\Delta_i||&=||v^*_{i-1}-v^*_i||\\
&=||J^{-1}(z_{i-1})\omega(z_{i-1})-J^{-1}(z_{i})\omega(z_{i})||\\
&=\left(L_\omega+\frac{1}{L_J}\right)max\left(\sigma_{max},\frac{1}{\sigma_{min}}\right)||z_i-z_{i-1}||\\
\end{align*}

We now expand $z_{i+1}$, and get:

\begin{align*}
||z_{i+1}-z_{i}||&=a_{i}||h(z_i)-J^T(z_{i})\bar v_i+M^z_{i+1}||
\end{align*}

Since $h(z_i)=\omega(z_i)+J^{-1}(z_{i})\omega(z_{i})$,

\[ ||h(z_i)||\le L_f+\frac{L_f}{\sigma_{min}} :=L_h \]

Further, on $G_n$, $||\bar v_i||<R^v_1$. Therefore:

\[ ||J^T(z_i)\bar v_i||\le \sigma_{max}R^v_1 \]

Letting $L^*=\left(L_\omega+\frac{1}{L_J}\right)max\left(\sigma_{max},\frac{1}{\sigma_{min}}\right)$, we have:

\[||\Delta_i||\le a_{i-1}L^*(L_h+\sigma_{max}R^v_1)+a_{i-1}L^*||M^z_i||\]

We now rewrite the term in \eqref{term:t3v}. Using the assumption that $||M_{n+1}^z||\le c_z(1+||z_n||)$: we get, that on $G_n$:

\[||\Delta_i||\le a_{i-1}(L^*(L_h+\sigma_{max}R^v_1)+L^*c_1(1+R^z+||z^*||)\]

Letting, $L_\Delta=L^*(L_h+\sigma_{max}R^v_1)+L^*c_z(1+R^z+||z^*||$:

\begin{align*} \left\Vert\sum_{i=n_0}^{n_1-2}\left(\prod_{j=i+1}^{n_1-1}B(z_j)\right)\Delta_{i+1}\right\Vert&\le L_\Delta \sum_{i=n_0}^{n_1-2} a_i \left\Vert\left(\prod_{j=i+1}^{n_1-1}B(z_j)\right)\right\Vert\\
&\le L_\Delta \sum_{i=n_0}^{n_1-2} \frac{a_i}{b_{i+1}} \left\Vert\left(b_{i+1}\prod_{j=i+1}^{n_1-1}B(z_j)\right)\right\Vert\\
\end{align*}


We note that $\left\Vert\left(\prod_{j=i+1}^{n_1-1}B(z_j)\right)\right\Vert \le \prod_{j=i+1}^{n_1-1}\delta_j$. Using that fact that $b_{i+1}\prod_{j=i+1}^{n_1-1}\delta_j\le \frac{1}{\sigma^2_{max}}$, we finally get that:

\[\left\Vert\sum_{i=n_0}^{n_1-2}\left(\prod_{j=i+1}^{n_1-1}B(z_j)\right)\Delta_{i+1}\right\Vert\le \frac{L_\Delta}{\sigma^2_{max}} \sup_{i\in [n_0,n_1]} \frac{a_i}{b_{i+1}}\]

Putting these together, and letting $\sum_{i=n_0}^{n_1-1}b_i\left(\prod_{j=i+1}^{n_1-1}B(z_j) \right)M^v_{i+1}:=S_v(n_0,n_1)$ we get that:
\begin{align*}
||\bar v_{n_1}||\le&  R^v_0 \prod_{i=n_0}^{n_0+n} \delta_i\\
&+\frac{L_\Delta}{\sigma^2_{max}} \sup_{i\in [n_0,n_1]} \frac{a_i}{b_{i+1}}\\
&+||S_v(n_0,n_1)||\\
&+a_{n_1-1}L_\Delta
\end{align*}

Now, since $\lim_{i\rar \infty} \frac{a_i}{b_{i+1}}=0$, and choosing $n_0$ large enough that $\sup_{i\in [n_0,\infty)} \frac{a_i}{b_{i+1}}\le \frac{\epsilon \sigma^2_{max} }{4L_\Delta}$, and $n_1$ large enough such that $\prod_{i=n_0}^{n_0+n} \delta_i \le \frac{\epsilon}{4R^v_0 }$ and $a_{n_1-1}\le \frac{\epsilon}{4L_\Delta }$: we get that, on $G_{n_1}$:

\begin{align*}
||\bar v_{n_1}||\le \frac{3\epsilon}{4}+||S_v(n_0,n_1)||\\
\end{align*}

Now, we bound $||S_v(n_0,n_1)||$ using \tc{red}{CITE BORKAR CONC INEQ}. Note that $S_v(n_0,n_1)$  is a martingale and that $||b_i\prod_{j=i+1}^{n_1-1}B(z_j)||\le b_i exp(-\sigma^2_{max} \sum_{j=i+1}^{n_1-1}b_j):=A_{i,n}$. Further note that $\mathbb{E}[exp(||M^v_{n+1}||)|G_n,\mc{F}_n]\le exp(c_1(1+R^v_0)):=K_1$, $\sum_{j=i}^{n} A_{j,n}\le \frac{1}{\sigma_{max}^2}$, and $\max_{n_0\le k\le n}A_{k,n}=b_n$. Since all the conditions are satisfied, we have that:

\begin{align*}
Pr(||S_v(n_0,n_1)||\ge \epsilon/4)\le \begin{cases}2d^2exp(-\frac{c\epsilon^2}{d^3b_n}) \ \ &: \epsilon \in \left(0,\frac{K_1 d \sqrt{d}}{\sigma_{max}^2}\right)\\
2d^2exp(-\frac{c\epsilon}{d \sqrt{d}b_n}) &: \text{otherwise}\end{cases} 
\end{align*}

The desired result follows.
\end{proof}


We now bound the slow-varying process using Alekseev's formula, which allows us to treat the error from the fast-time scale and the noise as perturbations to the limiting ode, $\dot z=-h(z)$. To do so, we first define the object of our analysis, the linear interpolation of $z_n$. First, we define $t_n=\sum_{i=0}^n a_n$. Then the linear interpolated process $\bar z(t)$ for $t \in [t_n,t_{n+1}]$ is given by:

\[\bar z(t)=\bar z(t_n)+\frac{t-t_n}{a_n}(\bar z (t_{n+1})-\bar z (t_n)) \]

Note, that the linear interpolation agrees with the discrete process at $t_n$ for $n\ge0$.

Thus, for any $n \ge0$:

\begin{align*}
\bar z(t)&=\bar z(t_{n_0})-\sum_{k=n_0}^n a_k (h(\bar z(t_k))+J^T(\bar z(t_k))\bar v_k+M_k^z)\\
&=\bar z(t_{n_0})-\sum_{k=n_0}^n \int_{t_k}^{t_{k+1}} [h(\bar z(t_k))+J^T(\bar z(t_k))\bar v_k+M_k^z]ds\\
&=\bar z(t_{n_0})-\int_{t_{n_0}}^{t_{n}}[ ]h(\bar z(s))+g_1(s) +g_2(s)+g_3(s)] ds
\end{align*}

Where, for $t \in [t_n,t_{n+1}]$:
\begin{align}
g_1(t)&=h(\bar z(t_{n}))-h(\bar z(t))\\
g_2(t)&=J^T(z(t_{n}))\bar v_n\\
g_3(t)&=M^z_{n+1}
\end{align}

Now, let a solution to the limiting ode, $\dot z=-h(z)$, starting at $z_0$ from $t_0$ to $t$, be given by $z(t,t_0,z_0)$. Via Alekseev's formula, we can write"

\[\bar z(t)=z(t,t_{n_0},\bar z(t_{n_0}))+\int_{t_{n_0}}^t \Phi(t,s,\bar z(s))(g_1(s)+g_2(s)+g_3(s))ds\]

Where $\Phi(t,s,\bar z(s))$ is the fundamental matrix of $\dot y=Dh(z_(t),s,u_0)y$ for $t\ge0$ where $Dh$ is the Jacobian along the trajectory of $z(t)$. Note that $g_1(s)+g_2(s)+g_3(s)$ is piece-wise continuous. 

\[\bar z(t)=z(t,t_{n_0},\bar z(t_{n_0}))+\int_{t_{n_0}}^t \Phi(t,s,\bar z(s))(g_1(s)+g_2(s)+g_3(s))ds\]

We now rewrite this as:

\[\bar z(t_n)=z(t,t_{n_0},\bar z(t_{n_0}))+W_n+S_n^z+(\tilde S_n^z-S_n)+V_n+(\tilde V_n-V_n) \]

Where:
\[ W_n=\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}\Phi(t,s,\bar z(s))[h(\bar z(t_k))-h(\bar z(s)]ds\]

\[ S^z_n=\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}\Phi(t,s,\bar z(t_k))dsM^z_k\]
\[ \tilde S^z_n=\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}\Phi(t,s,\bar z(s))dsM^z_k\]
\[ V_n=\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}\Phi(t,s,\bar z(t_k))ds \bar v_{t_k}\]
\[\tilde V_n=\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}\Phi(t,s,\bar z(s))ds \bar v_{t_k}\]

We first derive a useful bound which will be useful in our further developments:

\begin{lemma}
There exists a positive constant $C_1$ depending on $\sigma_{max}, L_h,$ and $R_1^z$ such that:
\begin{align}
&\int_{t_k}^{t_{k+1}}e^{-\lambda(t_n-s)}||\bar z(s)-\bar z(t_k)||ds \le C_1 a_k^2e^{-\lambda(t_n-t_{k+1})}
\end{align}
\label{lemma:genbnd}
\end{lemma}

\begin{proof}

\begin{align*}
||\bz(s)-\bz(t_k)||&=\frac{s-t_k}{a_k}||\bz(t_{k+1})-\bz(t_k)||\\
&\le(s-t_k)||h(\bz(t_k))+J^T(\bz(t_k))\bar v_k+M_k^z||\\
&\le(s-t_k)(L_h+\sigma_{max}||\bar v_k||+||M_k^z||)\\
\end{align*}

Since $\int_{t_k}^{t_{k+1}}(s-t)e^{-\lambda(t_n-s)}ds\le a_k^2 e^{-\lambda(t_n-t_{k+1})}$:

\begin{align*}
\int_{t_k}^{t_{k+1}}&e^{-\lambda(t_n-s)}||\bar z(s)-\bar z(t_k)||ds\\
&\le a_k^2 e^{-\lambda(t_n-t_{k+1})} (L_h+\sigma_{max}||\bar v_k||+||M_k^z||)\\
\end{align*}
Now, remarking that on $G_n$, $||M_k^z||\le c_z(1+||\bz(t_k))||)\le c_z(1+R^1_z)$ and $||\bar v_k||\le R_v$ our result follows.
\end{proof}

We now derive a bound on $||W_n||$ using Lemma~\ref{lemma:genbnd}.

\begin{lemma}
There exists a positive constant $C_2$ depending on $C_1,K_2,L_h, \lambda$ such that:
\begin{align}
||W_n||\le C_2(\sup_{k\ge n_0}a_k) %(1+||M^z_k||+||\bar v_k||)
\end{align}
\label{lemma:Wbnd}
\end{lemma}

\begin{proof}
\begin{align*}
||W_n||&\le \sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}||\Phi(t_n,s,\bz(s))||h(\bz(t_k))-h(\bz(s))||ds\\
&\le L_h K_2 \sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}} e^{-\lambda(t_n-s)}||\bz(t_k)-\bz(s)||ds\\
&\le L_h K_2 C_1 \sum_{k=n_0}^{n-1}a_k^2 e^{-\lambda(t_n-t_{k+1})}\\
&\le L_h K_2 C_1 \sup_{k\ge n_0}a_k\sum_{k=n_0}^{n-1}a_ke^{-\lambda(t_n-t_{k+1})}\\
\end{align*}

Now, using the fact that $\sum_{k=n_0}^{n-1}a_ke^{-\lambda(t_n-t_{k+1})}\le \frac{1}{\lambda}$, the desired result follows.
\end{proof}

We now derive a bound on $||\tilde S^z_n-S^z_n||$ and $||\tilde V_n-V_n||$. 

\begin{lemma}
There exists a positive constant $C_3$ depending on $C_1,K_3,\lambda,R^z_1$ such that, on $G_n$:
\begin{align}
||\tilde S^z_n-S^z_n||&\le C_3 \sup_{k\ge n_0}a_k\\
\end{align}
\label{lemma:Sbnd}
\end{lemma}


\begin{proof}
\begin{align*}
||\tilde S^z_n-S^z_n||&\le\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}||\Phi(t_n,s,\bz(s))-\Phi(t_n,s,\bz(t_{k})||ds||M_{k+1}^z||  \\
&\le K_3 C_1 \sum_{k=n_0}^{n-1}a^2_kC_1||M_{k+1}^z||e^{-\lambda(t_n-t_{k+1})}\\
&\le K_3 C_1 c_z(1+R^1_z)\sup_{k\ge n_0}a_k\sum_{k=n_0}^{n-1}a_ke^{-\lambda(t_n-t_{k+1})}
\end{align*}
\end{proof}


\begin{lemma}
There exists a positive constant $C_4$ depending on $C_1,K_3,\lambda,R^v_1$ such that, on $G_n$:
\begin{align}
||\tilde V_n-V_n||&\le C_4 \sup_{k\ge n_0}a_k 
\end{align}
\label{lemma:Vbnd}
\end{lemma}

\begin{proof}
\begin{align*}
||\tilde V^z_n-V^z_n||&\le\sum_{k=n_0}^{n-1}\int_{t_k}^{t_{k+1}}||\Phi(t_n,s,\bz(s))-\Phi(t_n,s,\bz(t_{k})||ds||v_{k+1}||  \\
&\le K_3 C_1 R^v_1 \sum_{k=n_0}^{n-1}a^2_kC_1e^{-\lambda(t_n-t_{k+1})}\\
&\le K_3 C_1 R^v_1 \sup_{k\ge n_0}a_k\sum_{k=n_0}^{n-1}a_ke^{-\lambda(t_n-t_{k+1})}
\end{align*}

Where the second inequality follows by using the fact that, on $G_n$, $||\bar v_k||\le R_1^v$, and then using \tc{red}{BORthm3} and then Lemma~\ref{lemma:genbnd}. Now using the fact that $\sum_{k=n_0}^{n-1}a_ke^{-\lambda(t_n-t_{k+1})}\le \frac{1}{\lambda}$, the desired result follows.
\end{proof}

Now, recall that the event we would like to bound is: $\{||z_n-z^*||<\epsilon \forall n\ge n_1\}$ on the event $\{||z_{n_0}-z^*||\le R_0^z\}$. where $n_1>n_0$. W will construct an upper bound on the complement of this event using the bounds we have just constructed and the martingale concentration inequality used in Lemma \ref{lemma:vconc}.

\begin{lemma}
\label{lemma:event}
\[\mc{E}^c_z(n_1)\subseteq \left[ \bigcup_{n_0\le n \le n_1} \left(\{E_{n+1}>R^z_1-R^z_0 ,G_n\}\cup \{||\bar v_{n+1}||>R^v,G_n\}\right)\right]\cup \left[ \bigcup_{n\ge n_1+1}\{E^*_{n+1}>\epsilon_1,||v_{n+1}||>R^v,G_n\}\right]\]
\end{lemma}

\begin{proof}
Define:
\[\mc{E}_z(n_1):=\{||\bar z(t)-z^*||<\epsilon_1 \ \ \forall \  t\ge t_{n_1+1}\}\cap \{||\bar v_n||<R^v \ \ \forall \  n\ge n_1+1\} \]
\[ B_{R^z_1}(z^*):=\{z: ||z-z^*|| \le R^z_1\}\]
\[ B_{R^v}(0):=\{v: ||v|| \le R^v\}\]
\[ E_{n+1}:=\sup_{t \in [t_n, t_{n+1}]} || \bar z(t)-z(t,t_{n_0},\bar z(t_{n_0}))||\]
\[ E^*_{n+1}:=\sup_{t \in [t_n, t_{n+1}]} || \bar z(t)-z^*||\]
\[ G^z_n:=\{\bz(t) \in B_{R^z}(z^*) \ \forall t \in [t_{n_0},t_n]\}\]
\[ G^v_n:=\{\bar v_k \in B_{R^v}(0) ; k=n_0,...,n\}\]
\[ G^{gap}_n:=\{\sup_{n_0\le k \le n } E_{k+1} >R^z_1-R^z_0\}\]
\[ G_n=G^z_n \cap G^v_n\]
\[ D_n=G^{gap}_n \cap G^v_n\]


We would like to find a superset of $\mc{E}^c_z(n_1)$ where $n_1=n_0+N$. 

%First, note that $\mc{E}_z(n_1)=\bigcap_{n=n_1+1}^{\infty} \{ E^*_{n+1} \le \epsilon \}$. Therefore $\mc{E}^c_z(n_1)=\bigcup_{n=n_1+1}^{\infty} \{ E^*_{n+1} > \epsilon \}$. 

%Now, $\bigcup_{n=n_1+1}^{\infty} \{ E^*_{n+1} > \epsilon \} \subseteq G_{n_1}^c \cup \bigcup_{n=n_1+1}^{\infty} \{ E^*_{n+1} > \epsilon \}$


\[ \mc{E}^c_z(n_1)= (\mc{E}^c_z(n_1)\cap D_{n_1}^c)\cup(\mc{E}^c_z(n_1)\cap D_{n_1}) \subseteq D_{n_1}^c\cup(\mc{E}^c_z(n_1)\cap D_{n_1})\]

We first analyze $D_{n_1}^c$:
\begin{align*}
D_{n_1}^c&=(G^{gap}_{n_1})^c \cup (G^v_{n_1})^c\\
&=\{\sup_{n_0\le n \le n_1 }E_{n+1}>R^z_1-R^z_0\}\cup \{\sup_{n_0\le k\le n_1+1}||\bar v_k||>R^v\}\\
&=\left[(G^{gap}_{n_1})^c \cup (G^v_{n_1})^c\right] \cup \left[\left(G^{gap}_{n_1} \cap G^v_{n_1} \right) \cap \left(\{E_{n_1+1}>R^z_1-R^z_0\}\cup \{||\bar v_{n_1+1}||>R^v\}\right)\right]
\end{align*}

Doing this recursively, we get:

\begin{align*}
D_{n_1}^c&=\bigcup_{n_0\le n \le n_1}\left(G^{gap}_{n} \cap G^v_{n} \right) \cap \left(\{E_{n+1}>R^z_1-R^z_0\}\cup \{||\bar v_{n+1}||>R^v\}\right)
\end{align*}

Using the fact that $G^{gap}_n\subseteq G^z_n$: lets us write this as:

\begin{align*}
D_{n_1}^c&\subseteq\bigcup_{n_0\le n \le n_1}\left(G^{z}_{n} \cap G^v_{n} \right) \cap \left(\{E_{n+1}>R^z_1-R^z_0\}\cup \{||\bar v_{n+1}||>R^v\}\right)\\
&=\bigcup_{n_0\le n \le n_1} \left(\{E_{n+1}>R^z_1-R^z_0 ,G_n\}\cup \{||\bar v_{n+1}||>R^v,G_n\}\right)
\end{align*}

Now we analyze $(\mc{E}^c_z(n_1)\cap D_{n_1})$. Since $D_{n_1}\subseteq G_{n_1}$, we can expand this, and write:

\[ \mc{E}^c_z(n_1)\cap D_{n_1}\subseteq \mc{E}^c_z(n_1) \cap G_{n_1} = \bigcup_{n\ge n_1+1}\{E^*_{n+1}>\epsilon_1,||v_{n+1}||>\epsilon_2,G_n\}\]

Thus we have:

\[\mc{E}^c_z(n_1)\subseteq \left[ \bigcup_{n_0\le n \le n_1} \left(\{E_{n+1}>R^z_1-R^z_0 ,G_n\}\cup \{||\bar v_{n+1}||>R^v,G_n\}\right)\right]\cup \left[ \bigcup_{n\ge n_1+1}\{E^*_{n+1}>\epsilon_1,||v_{n+1}||>R^v,G_n\}\right]\]

\end{proof}























